Pretrained ViTs Yield Versatile Representations For Medical Images

Convolutional Neural Networks (CNNs) have reigned for a decade as the de facto approach to automated medical image diagnosis, pushing the state-of-the-art in classification, detection and segmentation tasks. Over the last years, vision transformers (ViTs) have appeared as a competitive alternative to CNNs, yielding impressive levels of performance in the natural image domain, while possessing several interesting properties that could prove beneficial for medical imaging tasks. In this work, we explore the benefits and drawbacks of transformer-based models for medical image classification. We conduct a series of experiments on several standard 2D medical image benchmark datasets and tasks. Our findings show that, while CNNs perform better if trained from scratch, off-the-shelf vision transformers can perform on par with CNNs when pretrained on ImageNet, both in a supervised and self-supervised setting, rendering them as a viable alternative to CNNs.

==> 6_conclusions_ECCV.tex <==
\section{Conclusion}
\label{conclusions}

In this work we show that \emph{vision transformers can reliably replace CNNs on medical 2D image classification if appropriate training protocols are employed.}
More precisely, ViTs reach the same level of performance as CNNs in an array of medical classification and segmentation tasks, but they require transfer learning to do so.
But since \textsc{ImageNet} pretraining is the standard approach for CNNs, this does not incur any additional cost in practice.
The best overall performance on medical imaging tasks is achieved using in-domain self-supervised pretraining, where ViTs show a small advantage over CNNs.
As the data size grows, this advantage is expected to grow as well, as observed by  \cite{caron2021emerging} and our own experiments.
Additionally, ViTs have a number of properties that make them attractive: they scale similarly to CNNs (or better), their lack of inductive bias, global attention and skip connections may improve performance, and their self-attention mechanism provides a clearer picture of saliency. 
From a practitioner's point of view, these benefits are compelling enough to 
explore the use of ViTs in the medical domain.
Finally, modern CNNs have been studied extensively for more than a decade, while the first pure vision transformer appeared less than two years ago -- the potential for ViTs to improve is considerable.






% Finally, to answer the question posed in the title: \emph{vanilla transformers can reliably replace CNNs on medical image tasks with little effort}. 
% More precisely, ViTs can reach the same level of performance as CNNs in small medical datasets, but require transfer learning in order to do so. However, using ImageNet pretrained weights is the standard approach for CNNs as well, so the switch to ViTs is trivial. 
% Furthermore, ViTs can outperform CNNs using SSL pre-training when working with limited number of samples, but only marginally. 
% As the number of samples grows, the margin between ViT and CNN is expected to grow as well.
% This equal or better performance comes with the additional benefit of built in high-resolution saliency maps that can be used to better understand the model's decisions.

% \moein{
% In this work, we conducted a series of medical image classification and segmentation tasks, covering major domains of medical image datasets, and showed that baseline vision transformers could readily replace the CNN counterparts. ViTs perform similarly when transfer learning is utilized in classification tasks and outperform CNNs in segmentation. We showed that ViT-based models exhibit properties that are especially interesting in the medical image domain: they benefit more from self-supervision and are more interpretable than CNNs, both of which being very useful in medical image tasks.

% From a practitioner's point of view, these benefits are compelling enough to switch from convolutional models to vision transformers, especially given that such a low cost switch only requires changing a single encoder without the need to perform extensive hyper-parameter search.
% }



% \kevin{add thoughts: the gap between ViTs and CNNs will grow. Rand init is of limited use - only when data is quite big. Mixed precision thing. SEG: This, is in alignment with previous works who have shown the superiority of ViTs for segmentation tasks and we can only expect the advances architectural choices and training protocols to make ViTs the obvious choice for segmentation tasks.}


